13C17O suggests gravitational instability in the HL Tau disc

We present the first detection of the 13C17O J=3-2 transition toward the HL Tau protoplanetary disc. We find significantly more gas mass (at least a factor of ten higher) than has been previously reported using C18O emission. This brings the observed total disc mass to 0.2 M, which we consider to be a conservative lower limit. Our analysis of the Toomre Q profile suggests that this brings the disc into the regime of gravitational instability. The radial region of instability (50-110 au) coincides with the location of a proposed planet-carved gap in the dust disc and a spiral in the gas. We, therefore, propose that if the origin of the gap is confirmed to be due to a forming giant planet, then it is likely to have formed via the gravitational fragmentation of the protoplanetary disc.

==> HL Tau MNRAS Letter resub/response.tex <==
Dear Editor,

We thank the reviewer for a constructive report that has improved the clarity of our manuscript.  We have implemented the changes suggested, and hope that you will consider the revised version for publication.  We have responded to the individual points in the report below.

Kind Regards,
Alice Booth & John Ilee

##############################################################################

The key point is the assumed CO abundance, which is a factor 5
lower than in some other works, thereby leading to gas masses a factor
5 higher. The authors justify this by referring to work by Bosman et 
al 2018 and Schwarz et al 2018. However, these works show that 
the CO abundance could be significantly dependent on the temperature
and on the ionization rate if, as suggested by Cleeves et al 2015,
cosmic rays are excluded from the disk by magnetic fields.

A lack of CO depletion would bring up the Toomre Q factor to a value
around 4-5, i.e. in the stable regime.

The authors should expose this uncertainty more clearly.

A: We have now included a new subsection (4.2) that discusses the impact of several of our assumptions on the derived gas mass.  We now explicitly state how our value would change under the assumption of a higher CO abundance and other important parameters / scenarios.

##############################################################################

A second point is the difference between the assumed radial
profile and the observed one. What can be the cause of such a difference ?

A: Section 3 now includes an explicit discussion on the nature of this deficit of emission.  In short, since it does not coincide with any other observed substructure in the disc, we believe it to be a effect of the high optical depth in the disc at these frequencies (measured to be tau ~ 8 by Carrasco-Gonzalez et al. 2019).

##############################################################################

Below are some issues that should also be cleared up, the first one
being very annoying, although most likely a typo.

1) The cited value in the text is 0.2 (+0.5,-0.6) solar mass for the
disk mass derived from 13C17O. This is in clear discrepancy with the
Figure 2, which rather suggest a mass of 0.15 - 0.25 solar mass.
Is there a missing 0 digit in the quoted errorbars ?

A: We apologise for the confusion, this was due to a typo (+0.5 -> +0.6).  The cited value now reads 0.2 (+0.6, -0.6), with the errors propagated from the uncertainty in the flux radial profile (which is large, ~30 per cent, see Figure 1d).  We have now more clearly stated the origin of these quoted errors.

##############################################################################

2) Page 3, first column, line 55 

A more explicit discussion of the conversion from 13C17O J=2-1 line
intensity to gas mass surface density would be desirable here.
It should include:
  -) the conversion from line intensity to upper level surface density
  -) the impact of the partition function
  -) the impact of the assumed abundances
This would allow the reader to follow much more easily the origin
of the error bars.

A: This was omitted due to space restrictions, but we are happy to provide further detail.  We have now included an expanded paragraph in the new Section 4.1 that fully describes the conversion from line intensity to gas mass surface density, including the relevant equation(s), allowing the effects of the parameters discussed above to be followed by the reader.

##############################################################################

The reference to Carney et al 2019 does not seem appropriate here
(that paper is about CH3OH and H2CO in HD163296).

A: Indeed Carney et al. discuss other molecules in other discs, but our methodology is identical (and we felt offered a very clear explanation). Since we now explicitly state our methodology, we have referenced the original relation from Remijan et al. 2003. 

##############################################################################

3) Section 4.1

Page 3, second column, line 37

A factor of 70 is very large. A more detailed comparison with
the analysis of Wu et al would be welcome to elucidate why such 
a major effect can be obtained from C18O measurements.

The authors should at least scale the Wu et al results to the
same CO abundance as used in this paper. Currently, there is a factor
5 difference between the respective assumptions. 

A: We have now significantly expanded our discussion involving the comparison of disc mass measurements in Section 5.1.  The large difference can be explained by the C18O emission being optically thick, which we now directly demonstrate is the case.  If we adopt the same CO abundance as Wu et al., our derived gas mass is still at least a factor of 10 higher than the mass obtained from C18O.  We have revised the abstract accordingly.   

##############################################################################

They should also indicate what is the expected C18O opacity from
their model.

A: Our modelling does not extend to full radiative transfer (which would require further observational data for the HL Tau disc), so we are unable to determine the opacity.  However, as discussed above, we demonstrate from the observations that the C18O is optically thick in Section 5.1.

##############################################################################

Also, the 0.2 solar mass is derived from a model profile which clearly
does not match the measured profile. What would be the total
disk mass using the measured profile instead of the model one ?
Would that (combined with a common assumption for the CO abundance)
bring the Wu et al result in agreement ?
  
The same comparison could be done in a forward way, by computing
the expected C18O line flux from the current model and comparing
it with the measured flux from Wu et al.
  
A: As we discuss above and in the revised manuscript, we do not believe the deficit of emission to be due to the presence of a gas gap.  Nevertheless, directly integrating the observed profile from Figure 2 would lead to a 40 per cent drop in total disc mass within 110au, which is still a factor 6 larger than Wu et al. using the same CO abundance.  

##############################################################################

Page 3, second column line 42

Tapia et al 2019 only derive a dust mass: they do not derive a gas-to-dust mass ratio. The corresponding sentence should be re-written to
make clear that the gas-to-dust ratio is derived using the
Tapia et al dust measurement and the new estimate of the gas mass.

A: Tapia et al. use a combined dust/gas evolutionary disc model to reproduce ALMA and VLA continuum profiles of the HL Tau disc.  They find that a dust mass of 4.8 x 10^-3 Msun within 100au is required, which with the gas mass of their model (0.23 Msun), corresponds to a dust-to-gas mass ratio of twice the ISM value (e.g. d/g ~ 0.02, g/d ~ 50).  Therefore our new gas mass estimate is not involved in the calculation of these numbers.  We have rewritten the first paragraph of Section 5.1 to state this more clearly.  

##############################################################################

Page 3, end of second column 

The small impact of selective photodissociation is negligible compared
to the strong assumption of a depletion of CO  in the disk. 

A: We have added that this is likely a smaller effect than the other assumptions to Section 4.2

##############################################################################

Typos:

Page 3, First column, Last line
  "where profile" ==> "where the profile"
  
Fixed.

==> response.tex <==
Dear Editor,

We thank the reviewer for a constructive report that has improved the clarity of our manuscript.  We have implemented the changes suggested, and hope that you will consider the revised version for publication.  We have responded to the individual points in the report below.

Kind Regards,
Alice Booth & John Ilee

##############################################################################

The key point is the assumed CO abundance, which is a factor 5
lower than in some other works, thereby leading to gas masses a factor
5 higher. The authors justify this by referring to work by Bosman et 
al 2018 and Schwarz et al 2018. However, these works show that 
the CO abundance could be significantly dependent on the temperature
and on the ionization rate if, as suggested by Cleeves et al 2015,
cosmic rays are excluded from the disk by magnetic fields.

A lack of CO depletion would bring up the Toomre Q factor to a value
around 4-5, i.e. in the stable regime.

The authors should expose this uncertainty more clearly.

A: We have now included a new subsection (4.2) that discusses the impact of several of our assumptions on the derived gas mass.  We now explicitly state how our value would change under the assumption of a higher CO abundance and other important parameters / scenarios.

##############################################################################

A second point is the difference between the assumed radial
profile and the observed one. What can be the cause of such a difference ?

A: Section 3 now includes an explicit discussion on the nature of this deficit of emission.  In short, since it does not coincide with any other observed substructure in the disc, we believe it to be a effect of the high optical depth in the disc at these frequencies (measured to be tau ~ 8 by Carrasco-Gonzalez et al. 2019).

##############################################################################

Below are some issues that should also be cleared up, the first one
being very annoying, although most likely a typo.

1) The cited value in the text is 0.2 (+0.5,-0.6) solar mass for the
disk mass derived from 13C17O. This is in clear discrepancy with the
Figure 2, which rather suggest a mass of 0.15 - 0.25 solar mass.
Is there a missing 0 digit in the quoted errorbars ?

A: We apologise for the confusion, this was due to a typo (+0.5 -> +0.6).  The cited value now reads 0.2 (+0.6, -0.6), with the errors propagated from the uncertainty in the flux radial profile (which is large, ~30 per cent, see Figure 1d).  We have now more clearly stated the origin of these quoted errors.

##############################################################################

2) Page 3, first column, line 55 

A more explicit discussion of the conversion from 13C17O J=2-1 line
intensity to gas mass surface density would be desirable here.
It should include:
  -) the conversion from line intensity to upper level surface density
  -) the impact of the partition function
  -) the impact of the assumed abundances
This would allow the reader to follow much more easily the origin
of the error bars.

A: This was omitted due to space restrictions, but we are happy to provide further detail.  We have now included an expanded paragraph in the new Section 4.1 that fully describes the conversion from line intensity to gas mass surface density, including the relevant equation(s), allowing the effects of the parameters discussed above to be followed by the reader.

##############################################################################

The reference to Carney et al 2019 does not seem appropriate here
(that paper is about CH3OH and H2CO in HD163296).

A: Indeed Carney et al. discuss other molecules in other discs, but our methodology is identical (and we felt offered a very clear explanation). Since we now explicitly state our methodology, we have referenced the original relation from Remijan et al. 2003. 

##############################################################################

3) Section 4.1

Page 3, second column, line 37

A factor of 70 is very large. A more detailed comparison with
the analysis of Wu et al would be welcome to elucidate why such 
a major effect can be obtained from C18O measurements.

The authors should at least scale the Wu et al results to the
same CO abundance as used in this paper. Currently, there is a factor
5 difference between the respective assumptions. 

A: We have now significantly expanded our discussion involving the comparison of disc mass measurements in Section 5.1.  The large difference can be explained by the C18O emission being optically thick, which we now directly demonstrate is the case.  If we adopt the same CO abundance as Wu et al., our derived gas mass is still at least a factor of 10 higher than the mass obtained from C18O.  We have revised the abstract accordingly.   

##############################################################################

They should also indicate what is the expected C18O opacity from
their model.

A: Our modelling does not extend to full radiative transfer (which would require further observational data for the HL Tau disc), so we are unable to determine the opacity.  However, as discussed above, we demonstrate from the observations that the C18O is optically thick in Section 5.1.

##############################################################################

Also, the 0.2 solar mass is derived from a model profile which clearly
does not match the measured profile. What would be the total
disk mass using the measured profile instead of the model one ?
Would that (combined with a common assumption for the CO abundance)
bring the Wu et al result in agreement ?
  
The same comparison could be done in a forward way, by computing
the expected C18O line flux from the current model and comparing
it with the measured flux from Wu et al.
  
A: As we discuss above and in the revised manuscript, we do not believe the deficit of emission to be due to the presence of a gas gap.  Nevertheless, directly integrating the observed profile from Figure 2 would lead to a 40 per cent drop in total disc mass within 110au, which is still a factor 6 larger than Wu et al. using the same CO abundance.  

##############################################################################

Page 3, second column line 42

Tapia et al 2019 only derive a dust mass: they do not derive a gas-to-dust mass ratio. The corresponding sentence should be re-written to
make clear that the gas-to-dust ratio is derived using the
Tapia et al dust measurement and the new estimate of the gas mass.

A: Tapia et al. use a combined dust/gas evolutionary disc model to reproduce ALMA and VLA continuum profiles of the HL Tau disc.  They find that a dust mass of 4.8 x 10^-3 Msun within 100au is required, which with the gas mass of their model (0.23 Msun), corresponds to a dust-to-gas mass ratio of twice the ISM value (e.g. d/g ~ 0.02, g/d ~ 50).  Therefore our new gas mass estimate is not involved in the calculation of these numbers.  We have rewritten the first paragraph of Section 5.1 to state this more clearly.  

##############################################################################

Page 3, end of second column 

The small impact of selective photodissociation is negligible compared
to the strong assumption of a depletion of CO  in the disk. 

A: We have added that this is likely a smaller effect than the other assumptions to Section 4.2

##############################################################################

Typos:

Page 3, First column, Last line
  "where profile" ==> "where the profile"
  
Fixed.
